Subgraph Federated Learning with Missing Neighbor Generation

Graphs have been widely used in data mining and machine learning due to their unique representation of real-world objects and their interactions. As graphs are getting bigger and bigger nowadays, it is common to see their subgraphs separately collected and stored in multiple local systems. Therefore, it is natural to consider the subgraph federated learning setting, where each local system holds a small subgraph that may be biased from the distribution of the whole graph. Hence, the subgraph federated learning aims to collaboratively train a powerful and generalizable graph mining model without directly sharing their graph data. In this work, towards the novel yet realistic setting of subgraph federated learning, we propose two major techniques: (1) FedSage, which trains a GraphSage model based on FedAvg to integrate node features, link structures, and task labels on multiple local subgraphs; (2) FedSage+, which trains a missing neighbor generator along FedSage to deal with missing links across local subgraphs. Empirical results on four real-world graph datasets with synthesized subgraph federated learning settings demonstrate the effectiveness and efficiency of our proposed techniques. At the same time, consistent theoretical implications are made towards their generalization ability on the global graphs.

==> theory.tex <==
\section{Implication on Generalization Bound}
\label{sec:thoery}
In this section, we provide a theoretical implication for the generalization of the proposed methods. To narrow the gap between the real setting and theoretical setting, we follow Graph Neural Tangent Kernel (GNTK)~\cite{dhpwx19} on the overparameterized GNN.

\paragraph{Setting.} Our explanation builds on a {\em simplified} setting, where we assume a GNN $f_{\rm GNN}$ with aggregation operations and fully-connected layers with ReLU activation in each aggregation operation. 
%with $L$ level of aggregation operations and $R$ fully-connected layers with ReLU activation in each aggregation operation.
The weights of $f_{\rm GNN}$, $W$ is i.i.d. sampled from a multivariate Gaussian distribution $ \mathcal{N}(0,I)$. Let $G=\{V,E\}$, $G^{\prime}=\{V^{\prime}, E^{\prime}\}$ denote two graphs with $|V|=n$, $|V^{\prime}|=n^{\prime}$. 

% A BLOCK operation in GNTK calculates 1) a covariance matrix $\mathbf{\Sigma}^{(l)}(G,G^{\prime}) \in \mathbb{R}^{n \times n^{\prime}}$; and 2) the intermediate kernel values $\mathbf{\Theta}^{(l)}(G,G^{\prime}) \in \mathbb{R}^{n \times n^{\prime}}$.

\begin{definition}[Informal version of GNTK~\cite{dhpwx19}] 
%For transformation $r\in[R]$, layer $l \in [L]$, and for $u\in V$, $u^\prime \in V^\prime$,
Considering training a overparameterized GNN $f_{\rm GNN}$ by gradient desent with infinitesimally small learning rate, the kernel matrix of GNTK  is defined as 
\begin{align*}
     \mathbf{H}(G,G^{\prime}) = 
     \mathbb{E}_{W\sim \mathcal{N}(0,I)}\left[\left<\frac{\partial f_{\rm GNN}(W,G)}{\partial W}, \frac{f_{\rm GNN}(W,G^{\prime})}{\partial W}\right> \right] \in \mathbb{R}^{n \times n^{\prime}}.
    %  =\sum_{u\in V, u^\prime \in V^\prime}\left [\mathbf{\Theta}^{(l)}_{(R)}(G,G^{\prime}) \right ]_{uu^\prime} 
\end{align*}
\end{definition}
We provide full expression of $\mathbf{H}$ in Appendix~\ref{app:theory}. $\mathbf{H}$ can be viewed as kernel matrix. The generalization ability in the NTK regime and depends on the kernel matrix. 

\begin{theorem}[Generalization bound~\cite{dhpwx19}]\label{thm:bound} Given $n$ training data ${(G_i,y_i)}^n_{i=1}$ drawn iid from distribution $\mathcal{D}$. Consider any loss function $l: \mathbb{R} \times \mathbb{R} \mapsto [0,1]$ that is 1-Lipschitz in the first argument such that $l(y,y)=0$. With ptobability at least $1-\sigma$ and constant $c\in(0,1)$, the population loss of GNTK predictor has a upper bound that
\begin{align*}
    L_{\mathcal{D}(f_{\rm{GNTK}})} = \mathbb{E}_{(G,y)\sim\mathcal{D}}[l(f_{\rm{GNTK}}(G),y)] = O\left(\frac{\sqrt{\mathbf{y}^\top \mathbf{H}^{(-1)}\mathbf{y}\cdot \rm{tr}(\mathbf{H})}}{n} + \sqrt{\frac{\log (1/\sigma)}{n}}\right),
\end{align*}
\end{theorem}

The following Lemma~\ref{lem:bound1} and \ref{lem:bound2} give the bounds for $\sqrt{\mathbf{y}^\top \mathbf{H}^{(-1)}\mathbf{y}}$ and $\rm{tr}(\mathbf{H})$.
\begin{lemma}[Bound on $\sqrt{\mathbf{y}^\top \mathbf{H}^{(-1)}\mathbf{y}}$]\label{lem:bound1} For each $i \in [n]$, if the labels ${y_i}_{i=1}^n$ satisfies 
\begin{align*}
    y_i = \alpha_1\sum_{u\in V}\langle \bar{h}_u^\top, \beta_1 \rangle + \sum_{l=1}^{\infty}\alpha_{2l}\sum_{u\in V} \langle \bar{h}_u^\top, \beta_{2l} \rangle^{2l},
\end{align*}
where $\bar{h}_u =  c_u\sum_{v\in \mathcal{N}(u)\cup\{u\}}h_v$, $\alpha \in \mathbb{R}$, and $\beta \in \mathbb{R}^d$. We have
\begin{align*}
    \sqrt{\mathbf{y}^\top \mathbf{H}^{(-1)}\mathbf{y}} \leq 2|\alpha_1|\|\beta_1\|_2 + \sum_{l=1}^{\infty}\sqrt{2\pi}(2l-1)|\alpha_{2l}|\|\beta_{2l}\|_2^{2l} = o(n)
\end{align*}
\end{lemma}

\begin{lemma}[Bound on $\rm{tr}(\mathbf{H})$]\label{lem:bound2} If $\forall |V_i|$ in all the graphs $G_i = \{V_i, E_i\}$ of training set are up-bounded by $N$. Let $n$ denote as the number of training samples. Then $\rm{tr}(\mathbf{H}) \leq O(nN^2)$.
\end{lemma}

Combining Theorem~\ref{thm:bound}, Lemma~\ref{lem:bound1} and \ref{lem:bound2}, we state the generalization bound to the number of samples to motivate the benefits of utilizing more data in FL.

\begin{theorem}\label{thm:main}
Under the assumption in Lemma~\ref{lem:bound1} and assuming $N=o(\sqrt{n})$, $c$ is a constent that $c\in (0,1)$ the generalization error of GNTK can be upper-bounded by
\begin{align*}
 L_{\mathcal{D}(f_{\rm{GNTK}})} = \mathbb{E}_{(G,y)\sim\mathcal{D}}[l(f_{\rm{GNTK}}(G),y)] \lesssim O(1/n^c)  
\end{align*}
\end{theorem}

\textit{Proof.}
Given $\sqrt{\mathbf{y}^\top \mathbf{H}^{(-1)}\mathbf{y}}\leq o(n)$, $\rm{tr}(\mathbf{H}) \leq O(nN^2)$, with the valid assumption that $N=o(\sqrt{n})$, it is easy to see that $ L_{\mathcal{D}(f_{\rm{GNTK}})} \lesssim O(1/n^c)$


\begin{conjecture}
Till now, we show the bound in the classical setting, while equivalent to using local update step $K=1$ in FL. We can extend it to multi-local updates and global average fashion using the technique in FL-NTK~\cite{hlsy21}. Thus, we make the implication that the generalization bound inversely proportional to the polynomial of training samples $n$ holds in FL with $K>1$.
\end{conjecture}
